Relational Mathematics Continued

This is in some sense an addendum to the book Relational Mathematics by the first-named author. It originated from work on diverse other topics during which a lot of purely relational results with broad applicability have been produced. These include results on domain construction with novel formulae for existential and inverse image, a relational calculus for binary mappings, and the development of a formally derived relational calculus of Kronecker-, strict fork-, and strict join-operators. The many visualizations in this report make it also a scrap- and picture book for examples.

==> PrivateLabelWrite.tex <==
\def \ PropNegDiag{2.1}
\def \ PropTwoMaps{2.2}
\def \ PropResiRules{3.1}
\def \ PropSyqAndOr{3.2}
\def \ FigSyq{3.1}
\def \ ThmCancelA{3.3}
\def \ ThmCancelB{3.4}
\def \ ThmCancelC{3.5}
\def \ PropSyqSurjFct{3.6}
\def \ PropSyqLub{4.1}
\def \ FigAtomSingle{4.1}
\def \ LemmaEpsSigma{4.2}
\def \ FigQuotPow{4.2}
\def \ PropQuotPow{4.3}
\def \ DefExImInverseIm{5.1}
\def \ PropExImagProps{5.2}
\def \ PropSingleInverse{5.3}
\def \ FigExImage{5.1}
\def \ PropThetaInverseTheta{5.4}
\def \ FigExImageSurjective{5.2}
\def \ FigExImageNonSurjective{5.3}
\def \ PropPowerRelProps{5.5}
\def \ PropRelVec{6.1}
\def \ PropIdentityPointfree{6.2}
\def \ PropBOTTOPPointfree{6.3}
\def \ FigTranspInPoints{6.1}
\def \ PropTranspositionPointfree{6.4}
\def \ DefKronForkJoin{7.1}
\def \ FigKroneckerOfMaps{7.1}
\def \ PropPiKrhoEquGeneral{7.2}
\def \ PropForkMapKron{7.3}
\def \ FigKroneckerOfMapsZierer{7.2}
\def \ PropForkMapKronZierer{7.4}
\def \ PropForkMapKronJules{7.5}
\def \ FigKroneckerOfMapsJules{7.3}
\def \ PropResiFork{7.6}
\def \ FigSumPowToPowProdGeneral{7.4}
\def \ AdditionSyqGeneralized{7.7}
\def \ FigSumPowToPowProd{7.5}
\def \ PropSumPowToPowProd{7.8}
\def \ PropNegBinOp{8.1}
\def \ FigBinMap{8.1}
\def \ DefBinOp{8.2}
\def \ LemSwap{8.3}
\def \ FigAssocLaw{8.2}
\def \ DefInverse{8.4}
\def \ FigHasInverses{8.3}
\def \ DefInvariant{8.5}
\def \ FigHasInvariants{8.4}
\def \ DefNeutral{8.6}
\def \ FigHasRightNeutral{8.5}
\def \ FigHasRightNeutralUgly{8.6}
\def \ FigTwoNeutral{8.7}
\def \ LeftRightNeutral{8.7}
\def \ FigDistribut{8.8}
\def \ DefDistr{8.8}
\def \ FigSubsetElement{9.1}
\def \ FigNegaDisjoint{9.2}
\def \ FigSumPowToPowProdOnX{9.3}
\def \ CorSumPowToPowProd{9.1}
\def \ FigSumPowToPowProdMatrix{9.4}
\def \ PropPowerMeet{9.2}
\def \ PropNonClassIntersection{9.3}
\def \ PropPiAndRhoAndMeetSurj{9.4}
\def \ FigJoinMeet{9.5}
\def \ FigJoinMeetA{9.6}
\def \ PropAbsorbAssoc{9.5}

